The Lynchpin of In-Memory Computing: A Benchmarking Framework for Vector-Matrix Multiplication in RRAMs

The Von Neumann bottleneck, a fundamental challenge in conventional computer architecture, arises from the inability to execute fetch and data operations simultaneously due to a shared bus linking processing and memory units. This bottleneck significantly limits system performance, increases energy consumption, and exacerbates computational complexity. Emerging technologies such as Resistive Random Access Memories (RRAMs), leveraging crossbar arrays, offer promising alternatives for addressing the demands of data-intensive computational tasks through in-memory computing of analog vector-matrix multiplication (VMM) operations. However, the propagation of errors due to device and circuit-level imperfections remains a significant challenge. In this study, we introduce MELISO (In-Memory Linear Solver), a comprehensive end-to-end VMM benchmarking framework tailored for RRAM-based systems. MELISO evaluates the error propagation in VMM operations, analyzing the impact of RRAM device metrics on error magnitude and distribution. This paper introduces the MELISO framework and demonstrates its utility in characterizing and mitigating VMM error propagation using state-of-the-art RRAM device metrics.

==> junk.tex <==
%The von-Neumann bottleneck represents a critical limitation in computer architecture, characterized by the inability to concurrently perform fetch and data operations due to a shared bus between processing and memory units. This bottleneck significantly restricts system performance, increases energy consumption, and imposes constraints on computational complexity. Emerging non-volatile memory technologies like Resistive Random Access Memories (RRAMs) based on crossbar arrays present a promising solution for the challenges of data-intensive, large-scale computational tasks via in-memory computing of analog vector matrix multiplication operations. However, propogation of errors caused by device and circuit level limitations is a critical concern for these systems. In this paper we propose  comprehensive benchmarking framework, an end-to-end VMM benchmarking frame-work for RRAMs, called MELISO - In-Memory Linear Solver, designed to provide a comprehensive analysis of the error propagation during VMM operations. We investigate the impact of RRAM device metrics and the magnitude and distribution of the errors generated.
